Privacy-Preserving In-Context Learning for Large Language Models

In-context learning (ICL) is an important capability of Large Language Models (LLMs), enabling these models to dynamically adapt based on specific, in-context exemplars, thereby improving accuracy and relevance. However, LLM's responses may leak the sensitive private information contained in in-context exemplars. To address this challenge, we propose Differentially Private In-context Learning (DP-ICL), a general paradigm for privatizing ICL tasks. The key idea for DP-ICL paradigm is generating differentially private responses through a noisy consensus among an ensemble of LLM's responses based on disjoint exemplar sets. Based on the general paradigm of DP-ICL, we instantiate several techniques showing how to privatize ICL for text classification and language generation. We evaluate DP-ICL on four text classification benchmarks and two language generation tasks, and our empirical results show that DP-ICL achieves a strong utility-privacy tradeoff.

==> figure/table_ablation_classify.tex <==
    
% \begin{table}[H]
%     \caption{ Results of DP-ICL for Text classification with GPT2 variants}
%          % \vspace{-4mm}
%     \centering
%     \resizebox{0.95\textwidth}{!}{%
%     \begin{tabular}{@{}clcccccc@{}}
%     \toprule
%     \textbf{Dataset} & \textbf{Model} & $\epsilon=0$ (0-shot)   & $\epsilon=1$ & $\epsilon=3$ & $\epsilon=8$ & $\epsilon=\infty$ (Agg)& $\epsilon=\infty $\\ \midrule
%    \multirow{3}{*}{SST-2} & GPT2-medium & 73.05 & 59.70$_{1.13}$ &   59.74$_{0.88}$ &   59.59$_{0.84}$ & 61.90$_{0.88}$ & 58.77$_{1.46}$ \\ 
%                           & GPT2-large  & 86.12 & 66.57$_{1.55}$ &   69.30$_{1.28}$ &   69.85$_{1.34}$ & 73.05$_{1.55}$ & 62.63$_{1.58}$\\
%                           & GPT2-xl     & 73.97 & 62.46$_{0.95}$ &   61.18$_{0.81}$ &   60.87$_{0.78}$ & 63.17$_{0.98}$ & 64.50$_{1.11}$\\ \midrule
%    \multirow{3}{*}{Amazon}& GPT2-medium & 78.30  & 86.15$_{0.52}$ &   86.21$_{0.49}$ &   86.21$_{0.52}$ & 85.10$_{0.37}$ & 84.72$_{0.72}$ \\ 
%                           & GPT2-large  & 95.00 & 90.68$_{0.60}$ &   91.28$_{0.53}$ &   91.45$_{0.53}$ & 90.96$_{0.53}$ & 84.04$_{0.94}$\\
%                           & GPT2-xl     & 80.80 & 70.95$_{0.62}$ &   70.90$_{0.58}$ &   70.87$_{0.55}$ & 67.92$_{0.28}$ & 71.32$_{0.87}$\\ \midrule
%    \multirow{3}{*}{AGNews}& GPT2-medium & 55.80 & 50.37$_{1.33}$ &   55.16$_{1.09}$ &   55.92$_{1.07}$ & 56.66$_{0.99}$ & 46.40$_{1.28}$ \\ 
%                           & GPT2-large  & 59.50 & 43.99$_{1.36}$ &   49.55$_{1.39}$ &   50.96$_{1.39}$ & 52.22$_{1.06}$ & 40.70$_{1.47}$\\
%                           & GPT2-xl     & 66.70 & 52.99$_{1.85}$ &   59.65$_{2.40}$ &   61.05$_{2.70}$ & 64.50$_{2.82}$ & 47.10$_{3.86}$\\ \midrule
%    \multirow{3}{*}{TREC}  & GPT2-medium & 10.20 & 23.84$_{1.63}$ &   27.57$_{1.40}$ &   28.10$_{1.40}$ & 28.24$_{1.13}$ & 24.94$_{1.63}$ \\ 
%                           & GPT2-large  & 8.00 & 24.18$_{1.69}$ &   27.67$_{1.38}$ &   28.00$_{1.40}$ & 27.64$_{1.51}$ & 26.97$_{1.57}$\\
%                           & GPT2-xl     & 15.60 & 19.92$_{1.25}$ &   18.45$_{0.83}$ &   17.90$_{0.76}$ & 17.16$_{0.59}$ & 21.35$_{1.31}$ \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \label{tab:abl_classify_model}
%     \end{table}



% \begin{table}[H]
%     \caption{ Results of DP-ICL for Text classification with GPT2 variants}
%          % \vspace{-4mm}
%     \centering
%     \resizebox{0.85\textwidth}{!}{%
%     \begin{tabular}{@{}clccccc@{}}
%     \toprule
%     \textbf{Dataset} & \textbf{Model}    & $\epsilon=1$ & $\epsilon=3$ & $\epsilon=8$ & $\epsilon=\infty$ (Agg)& $\epsilon=\infty $\\ \midrule
%    \multirow{3}{*}{SST-2} & GPT2-medium  & 59.70$_{1.13}$ &   59.74$_{0.88}$ &   59.59$_{0.84}$ & 61.90$_{0.88}$ & 58.77$_{1.46}$ \\ 
%                           & GPT2-large  & 66.57$_{1.55}$ &   69.30$_{1.28}$ &   69.85$_{1.34}$ & 73.05$_{1.55}$ & 62.63$_{1.58}$\\
%                           & GPT2-xl     & 62.46$_{0.95}$ &   61.18$_{0.81}$ &   60.87$_{0.78}$ & 63.17$_{0.98}$ & 64.50$_{1.11}$\\ \midrule
%    \multirow{3}{*}{Amazon}& GPT2-medium   & 86.15$_{0.52}$ &   86.21$_{0.49}$ &   86.21$_{0.52}$ & 85.10$_{0.37}$ & 84.72$_{0.72}$ \\ 
%                           & GPT2-large  & 90.68$_{0.60}$ &   91.28$_{0.53}$ &   91.45$_{0.53}$ & 90.96$_{0.53}$ & 84.04$_{0.94}$\\
%                           & GPT2-xl     & 70.95$_{0.62}$ &   70.90$_{0.58}$ &   70.87$_{0.55}$ & 67.92$_{0.28}$ & 71.32$_{0.87}$\\ \midrule
%    \multirow{3}{*}{AGNews}& GPT2-medium  & 50.37$_{1.33}$ &   55.16$_{1.09}$ &   55.92$_{1.07}$ & 56.66$_{0.99}$ & 46.40$_{1.28}$ \\ 
%                           & GPT2-large   & 43.99$_{1.36}$ &   49.55$_{1.39}$ &   50.96$_{1.39}$ & 52.22$_{1.06}$ & 40.70$_{1.47}$\\
%                           & GPT2-xl     & 52.99$_{1.85}$ &   59.65$_{2.40}$ &   61.05$_{2.70}$ & 64.50$_{2.82}$ & 47.10$_{3.86}$\\ \midrule
%    \multirow{3}{*}{TREC}  & GPT2-medium & 23.84$_{1.63}$ &   27.57$_{1.40}$ &   28.10$_{1.40}$ & 28.24$_{1.13}$ & 24.94$_{1.63}$ \\ 
%                           & GPT2-large  & 24.18$_{1.69}$ &   27.67$_{1.38}$ &   28.00$_{1.40}$ & 27.64$_{1.51}$ & 26.97$_{1.57}$\\
%                           & GPT2-xl    & 19.92$_{1.25}$ &   18.45$_{0.83}$ &   17.90$_{0.76}$ & 17.16$_{0.59}$ & 21.35$_{1.31}$ \\
%     \bottomrule
%     \end{tabular}%
%      }
%     \label{tab:abl_classify_model}
%     \end{table}

==> figure/table_ablation_classify2.tex <==
    
\begin{table}[H]
    \caption{ Results of DP-ICL for Text classification with GPT2 variants}
         % \vspace{-4mm}
    \centering
    \resizebox{0.95\textwidth}{!}{%
    \begin{tabular}{@{}clcccccc@{}}
    \toprule
    \textbf{Dataset} & \textbf{Model} & $\epsilon=0$ (0-shot)   & $\epsilon=1$ & $\epsilon=3$ & $\epsilon=8$ & $\epsilon=\infty$ (Agg)& $\epsilon=\infty $\\ \midrule
   \multirow{3}{*}{SST-2} & GPT2-medium & 73.05 & 77.16$_{1.11}$ &   77.68$_{1.08}$ &   77.89$_{1.05}$ & 77.39$_{0.88}$ & 66.51$_{1.44}$ \\ 
                          & GPT2-large  & 86.12 & 56.95$_{1.30}$ &   57.18$_{1.34}$ &   57.25$_{1.26}$ & 56.83$_{0.82}$ & 53.78$_{1.58}$\\
                          & GPT2-xl     & 73.97 & 69.57$_{0.95}$ &   69.54$_{0.94}$ &   69.59$_{0.95}$ & 73.90$_{0.91}$ & 68.32$_{1.32}$\\ \midrule
   \multirow{3}{*}{Amazon}& GPT2-medium & 78.30 & 77.27$_{1.09}$ &   77.77$_{1.05}$ &   77.91$_{1.05}$ & 78.62$_{0.79}$ & 66.51$_{1.45}$ \\ 
                          & GPT2-large  & 95.00 & 90.68$_{0.60}$ &   91.28$_{0.53}$ &   91.45$_{0.53}$ & 90.96$_{0.53}$ & 84.04$_{0.94}$\\
                          & GPT2-xl     & 80.80 & 70.95$_{0.62}$ &   70.90$_{0.58}$ &   70.87$_{0.55}$ & 67.92$_{0.28}$ & 71.32$_{0.87}$\\ \midrule
   \multirow{3}{*}{AGNews}& GPT2-medium & 55.80 & 50.37$_{1.33}$ &   55.16$_{1.09}$ &   55.92$_{1.07}$ & 56.66$_{0.99}$ & 46.40$_{1.28}$ \\ 
                          & GPT2-large  & 59.50 & 43.99$_{1.36}$ &   49.55$_{1.39}$ &   50.96$_{1.39}$ & 52.22$_{1.06}$ & 40.70$_{1.47}$\\
                          & GPT2-xl     & 66.70 & 52.99$_{1.85}$ &   59.65$_{2.40}$ &   61.05$_{2.70}$ & 64.50$_{2.82}$ & 47.10$_{3.86}$\\ \midrule
   \multirow{3}{*}{TREC}  & GPT2-medium & 10.20 & 23.84$_{1.63}$ &   27.57$_{1.40}$ &   28.10$_{1.40}$ & 28.24$_{1.13}$ & 24.94$_{1.63}$ \\ 
                          & GPT2-large  & 8.00 & 24.18$_{1.69}$ &   27.67$_{1.38}$ &   28.00$_{1.40}$ & 27.64$_{1.51}$ & 26.97$_{1.57}$\\
                          & GPT2-xl     & 15.60 & 19.92$_{1.25}$ &   18.45$_{0.83}$ &   17.90$_{0.76}$ & 17.16$_{0.59}$ & 21.35$_{1.31}$ \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:abl_classify_model_1shot}
    \end{table}

==> figure/table_gen_ocr.tex <==


    
\begin{table}[H]
    \caption{ Results of DP-ICL for Document Visual Question Answering}
         % \vspace{-4mm}
    \centering
    \resizebox{0.95\textwidth}{!}{%
    \begin{tabular}{@{}cccccccc@{}}
    \toprule
    \textbf{Methods} & \textbf{Metrics} & $\epsilon=0$ (0-shot)   & $\epsilon=1$ & $\epsilon=3$ & $\epsilon=8$ & $\epsilon=\infty$ (Agg)& $\epsilon=\infty $\\ \midrule
   \multirow{3}{*}{Embedding} 
   & ROUGE-1     & 49.64 & tbd &   tbd &   tbd &  & 74.38 \\ 
   & BLEU        & 23.00 & tbd &   tbd &   tbd &  & 47.25 \\
   & Levenshtein & 38.99 & tbd &   tbd &   tbd &  & 69.37 \\ 
  \midrule
   \multirow{3}{*}{Key Word} 
   & ROUGE-1     & 49.64 & tbd &   tbd &   tbd &  & 74.38 \\ 
   & BLEU        & 23.00 & tbd &   tbd &   tbd &  & 47.25 \\
   & Levenshtein & 38.99 & tbd &   tbd &   tbd &  & 69.37 \\ 
    \bottomrule
    \end{tabular}%
    }
    \label{tab:gen_ocr_main}
    \end{table}

==> sections/prel.tex <==


\section{Background and Preliminaries}
\label{sec:pre}
We present an overview of in-context learning and provide a primer on the multiple associated concepts of differential privacy. Alongside each concept we provide intuition for the corresponding guarantees and limitations of our system.


\textbf{In-Context Learning.}
To answer a query $Q$ with ICL, we concatenate a sequence of $k$ exemplars (i.e., query-answer pairs) $S := \left( (Q_1,A_1), (Q_2,A_2), \ldots, (Q_k,A_k) \right)$ to $Q$ using an appropriate format and instructions. We then use the LLM to generate the next token via $\argmax_A \LLM(A|S + Q)$, where $+$ denotes concatenation. Intuitively, exemplars assist the LLM in identifying the relevant mapping between $(Q, A)$, which substantially enhances performance compared to directly querying test data, also known as zero-shot learning. 


\textbf{Differential Privacy.} 
Differential privacy \citep{dwork2006calibrating} is the gold standard for reasoning about the privacy of machine learning algorithms.
Formally, we call a randomized algorithm $\M$ is $(\eps, \delta)$-differentially private if it follows $\Pr[\M(D) \in E] \le e^\eps\cdot \Pr[\M(D') \in E] + \delta \nonumber$, where adjacent dataset $D$ and $D'$ only differ in one data point. 
It indicates that if two datasets are similar, a DP algorithm should produce similar output $E$ with a high probability so that attackers cannot infer the difference between them. 


In our case, $\M$ functions as an in-context learning (ICL) algorithm, producing answers to queries by utilizing private data as in-context exemplars. If this ICL algorithm adheres to differential privacy, it should generate similar outputs even when the in-context exemplars vary. Consequently, this prohibits the generation of private information, such as replicating the in-context exemplars, like Figure \ref{Fig:privacyattack}.

%


% % \tianhao{only keep a small piece of background}

% % \tianhao{In this work, we assume that each user can make a finite number of queries. 
% % % , that can be unrestricted in content, and can only observe the API's output. 
% % We further assume that the users do not collude. 
% % % Consequently, an attacker can employ various attack vectors, including but not limited to prompt leaking~\citep{perez2022ignore}. Given the rapidly evolving nature of LLM attacks, a priority for designing defenses is to ensure they are \emph{future-proof}. In other words, an organization seeking a solution to implement alongside their private data-augmented LLM should not have to worry about the defense being easily overcome by an adaptive attacker.
% % }

% % \begin{remark}[Assumption of a bounded number of queries the adversary can make]
% % We argue that the private querying system and attacker described in our threat model capture the essential security considerations for real-world deployments. The programmatic separation between analyst and query-answerer is implemented in the federated DP deployments surveyed in \citet{garrido2022lessons, salildont}. In our system, ICL serves as a tool for answering private queries while maintaining data privacy. The attacker's abilities and limitations are also realistic: API rate limits stem from hardware constraints, and since organizations store user queries for security purposes \citep{openai_2023}, attackers cannot expect unlimited attempts to extract private information.
% % \end{remark}


% We present an overview of in-context learning and provide a primer on the multiple associated concepts of differential privacy. Alongside each concept we provide intuition for the corresponding guarantees and limitations of our system.




% We use $D, D' \in \cup_{n \in \mathbb{N}} \cX^n$ to denote two datasets with an unspecified size over space $\cX$. We call two datasets $D$ and $D'$ \emph{adjacent} (denoted as $D \sim D'$) if we can construct one by adding/removing one data point from the other.

% \begin{definition}[Differential Privacy \citep{dwork2006calibrating}] 
% \label{def:DP}
% For $\eps, \delta \ge 0$, a randomized algorithm $\M : \MS(\cX) \rightarrow \cY$ is 
% {\em $(\eps, \delta)$-differentially private} if for every pair of adjacent datasets $D, D'\in \MS(\cX)$ and for every subset of possible outputs $E \subseteq \cY$, 
% \begin{equation}
% \Pr[\M(D) \in E] \le e^\eps\cdot \Pr[\M(D') \in E] + \delta \nonumber
% \end{equation}
% where the randomness is over the coin flips of $\M$. 
% \end{definition}

% Thus, differential privacy requires that for all adjacent datasets $D, D'$, the output distribution $\M(D)$ and $\M(D')$ are close, where the closeness is measured by the parameters $\eps$ and $\delta$. 

% In our case, $\M$ is an in-context learning algorithm that outputs an answer to a query by using exemplars. 
% A critical observation is that the DP guarantee is agnostic to the attacker's knowledge about DP algorithm $\M$ (except for the randomness being used in the execution). 
% That is, our guarantee is \emph{future-proof}: a DP-ICL system deployed years from now will provide the same guarantees even if attackers use adaptive attacks that may be invented in the future.
% The parameter $\eps$ is a `privacy budget': as $\eps$ increases, our method is able to give answers that reveal more information about the exemplars.
% Note that $\eps$ is an \emph{exponential} parameter: the attacker's increase in knowledge is bounded by $e^\eps$, so a privacy guarantee of $e^3$ is $e^5 \approx 150 \times$ `stronger' than a privacy guarantee of $e^8$.


==> sections/privacyanalysis.tex <==
\section{Privacy Analysis}


\tong{I put the previous privacy analysis in Appendix \ref{appendix_privacyanalysis}}
